Employing Deep Ensemble Learning for Improving the Security of Computer Networks against Adversarial Attacks

In the past few years, Convolutional Neural Networks (CNN) have demonstrated promising performance in various real-world cybersecurity applications, such as network and multimedia security. However, the underlying fragility of CNN structures poses major security problems, making them inappropriate for use in security-oriented applications including such computer networks. Protecting these architectures from adversarial attacks necessitates using security-wise architectures that are challenging to attack. In this study, we present a novel architecture based on an ensemble classifier that combines the enhanced security of 1-Class classification (known as 1C) with the high performance of conventional 2-Class classification (known as 2C) in the absence of attacks.Our architecture is referred to as the 1.5-Class (SPRITZ-1.5C) classifier and constructed using a final dense classifier, one 2C classifier (i.e., CNNs), and two parallel 1C classifiers (i.e., auto-encoders). In our experiments, we evaluated the robustness of our proposed architecture by considering eight possible adversarial attacks in various scenarios. We performed these attacks on the 2C and SPRITZ-1.5C architectures separately. The experimental results of our study showed that the Attack Success Rate (ASR) of the I-FGSM attack against a 2C classifier trained with the N-BaIoT dataset is 0.9900. In contrast, the ASR is 0.0000 for the SPRITZ-1.5C classifier.

==> Acknowledgment.tex <==
\section*{Acknowledgments}
\label{Acknowledgments}
This work is funded by the University of Padua, Italy, under the STARS Grants program (Acronym and title of the project: LIGHTHOUSE: Securing the Transition Toward the Future Internet).

==> IEEE_TNSM_Template.tex <==
% The paper headers
\markboth{Journal of \LaTeX\ Class Files,~Vol.~14, No.~8, August~2015}%
{Shell \MakeLowercase{\textit{et al.}}: Bare Demo of IEEEtran.cls for IEEE Communications Society Journals}

\appendices
\section{Proof of the First Zonklar Equation}
Appendix one text goes here.

% you can choose not to have a title for an appendix
% if you want by leaving the argument blank
\section{}
Appendix two text goes here.


% use section* for acknowledgment
\section*{Acknowledgment}


The authors would like to thank...


% Can use something like this to put references on a page
% by themselves when using endfloat and the captionsoff option.
\ifCLASSOPTIONcaptionsoff
  \newpage
\fi



% trigger a \newpage just before the given reference
% number - used to balance the columns on the last page
% adjust value as needed - may need to be readjusted if
% the document is modified later
%\IEEEtriggeratref{8}
% The "triggered" command can be changed if desired:
%\IEEEtriggercmd{\enlargethispage{-5in}}

% references section

% can use a bibliography generated by BibTeX as a .bbl file
% BibTeX documentation can be easily obtained at:
% http://mirror.ctan.org/biblio/bibtex/contrib/doc/
% The IEEEtran BibTeX style support page is at:
% http://www.michaelshell.org/tex/ieeetran/bibtex/
%\bibliographystyle{IEEEtran}
% argument is your BibTeX string definitions and bibliography database(s)
%\bibliography{IEEEabrv,../bib/paper}
%
% <OR> manually copy in the resultant .bbl file
% set second argument of \begin to the number of references
% (used to reserve space for the reference number labels box)
\begin{thebibliography}{1}

\bibitem{IEEEhowto:kopka}
H.~Kopka and P.~W. Daly, \emph{A Guide to \LaTeX}, 3rd~ed.\hskip 1em plus
  0.5em minus 0.4em\relax Harlow, England: Addison-Wesley, 1999.

\end{thebibliography}

% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:

\begin{IEEEbiography}{Michael Shell}
Biography text here.
\end{IEEEbiography}

% if you will not have a photo at all:
\begin{IEEEbiographynophoto}{John Doe}
Biography text here.
\end{IEEEbiographynophoto}

% insert where needed to balance the two columns on the last page with
% biographies
%\newpage

\begin{IEEEbiographynophoto}{Jane Doe}
Biography text here.
\end{IEEEbiographynophoto}

% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}



% that's all folks

==> Notes.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In the cross model transferability, the attacks can be transferred between the classifiers. Concretely, the adversary uses the victim model as an oracle, then queries the oracle repeatedly for the decisions on how the model will classify the data. These decisions are trained separately on a complete different model, which eventually generates the adversarial example.





MSI GF65 THIN 
Cry7 10 generation
GPU: Nvidea Gforce 2060Ti
32GB


==> PLAN.tex <==
1-Page Limit
2-Table 4

3-Why we applied the 

==> Tables/Accuracy.tex <==
%\begin{table}[!h]
%\scriptsize
%\centering
%\caption{Summary of the accuracies achieved for the considered networks with their Respective Datasets.\label{Accuracy}}
%\begin{tabular}{|p{1cm}|c|c|c|}
%\hline
%\textbf{Network} & $N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ1}^{DGA}$ & $N_{SPRITZ2}^{N-BaIoT}$ \TBstrut\\ %\hline
%
%\textbf{Accuracy} & 99.80\% & 99.50\% & 99.80\%  %\TBstrut\\\hline
%
%\textbf{Network} & $N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ1}^{RIPE}$ & $N_{SPRITZ2}^{RIPE}$ \TBstrut\\ \hline
%
%\textbf{Accuracy} & 99.80\% & 99.20\% & 99.80\%  %\TBstrut\\\hline
%
%\end{tabular}
%\end{table}

==> Tables/Cases.tex <==
\begin{table}[!h]

%\scriptsize
\centering
\caption{Scenarios of the Considered Source and Target Networks.\label{Cases}}
\begin{threeparttable}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\backslashbox{\textbf{SN}}{\textbf{TN}} & \bm{$N_{1}$}  & \bm{$N_{2}$} & \bm{$N_{3}$} & \bm{$N_{4}$} & \bm{$N_{5}$} & \bm{$N_{6}$} \\ \hline

\bm{$N_{1}$} & \cellcolor{grey} & CT &  CM &   CMT & CT& \cellcolor{grey} \TBstrut\\\hline

\bm{$N_{2}$} &  CT &  \cellcolor{grey}& \cellcolor{grey} &   CM &\cellcolor{grey}&\cellcolor{grey}\TBstrut\\\hline

\bm{$N_{3}$} &  CM  & \cellcolor{grey} & \cellcolor{grey} &   CT &\cellcolor{grey}&\cellcolor{grey} \TBstrut\\\hline

\bm{$N_{4}$ }&  CMT  &  CM  &  CT & \cellcolor{grey} &\cellcolor{grey}&\cellcolor{grey}\TBstrut\\\hline

\bm{$N_{5}$} & \cellcolor{grey} &  \cellcolor{grey}  & \cellcolor{grey} & \cellcolor{grey} &\cellcolor{grey}&CM\TBstrut\\\hline

\bm{$N_{6}$} & \cellcolor{grey}  &  \cellcolor{grey}  & \cellcolor{grey} & \cellcolor{grey} &\cellcolor{grey}&CMT\TBstrut\\\hline


\end{tabular}

\begin{tablenotes}
      \small
      \item \small
    \bm{$N_{1}$}:$N_{SPRITZ1}^{N-BaIoT}$, \bm{$N_{2}$}:$N_{SPRITZ1}^{DGA}$, \bm{$N_{3}$}:$N_{SPRITZ2}^{N-BaIoT}$,  
\end{tablenotes}

\begin{tablenotes}
      \small
      \item \small \bm{$N_{4}$}:$N_{SPRITZ2}^{DGA}$ \bm{$N_{5}$}:$N_{SPRITZ1}^{RIPE}$,  \bm{$N_{6}$}:$N_{SPRITZ2}^{N-RIPE}$
    
\end{tablenotes}
\end{threeparttable}
%\begin{tablenotes}
 %     \small
  %  $N_{1}$:$N_{SPRITZ1}^{N-BaIoT}$, %$N_{2}$:$N_{SPRITZ1}^{DGA}$, $N_{3}$:$N_{SPRITZ2}^{N-BaIoT}$, %$N_{4}$:$N_{SPRITZ2}^{DGA}$, $N_{5}$:$N_{SPRITZ1}^{RIPE}$,  %$N_{6}$:$N_{SPRITZ2}^{N-RIPE}$
   % \end{tablenotes}

\end{table}


==> Tables/CrossModel/CM_BaIoT_First.tex <==
\begin{table*}[!h]
%\scriptsize
\centering
\caption{Experimental Results for Cross Model Transferability on N-BaIoT and DGA datasets\\ (SPRITZ1 and SPRITZ2 are used interchangeably in the SN an the TN). \label{CM_BaIoT_First}}
\resizebox{2\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{SN} & \textbf{TN} & \textbf{Accuracy} & \textbf{Attack Type} & \textbf{PSNR} & \textbf{$L_1$ dist} & \textbf{Max. dist} & \textbf{ASR} & \textbf{ASR} \TBstrut\\
& & & & & & & \textbf{(SN)} & \textbf{(TN)}  \\ \hline
 \rowcolor{grey}
$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ2}^{N-BaIoT}$ & SN = 98.90\% , TN = 98.80\% & I-FGSM, $\varepsilon$ = 0.1 & 18.65 & 22.07 & 64.78  & 1.0000 & 0.0030 \TBstrut\\ \hline

$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ2}^{N-BaIoT}$ & SN = 98.90\% , TN = 98.80\% & I-FGSM, $\varepsilon$ = 0.01 & 18.93 & 21.26 & 62.71  & 1.0000 & 0.0000 \TBstrut\\ \hline
 \rowcolor{grey}
$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ2}^{N-BaIoT}$ & SN = 98.90\% , TN = 98.80\% & I-FGSM, $\varepsilon$ = 0.001 &  19.04 & 20.94 & 61.76  & 1.0000 & 0.0000 \TBstrut\\ \hline

$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ2}^{N-BaIoT}$ & SN = 98.90\% , TN = 98.80\% & \textbf{JSMA, $\theta$ = 0.1} & \textbf{18.49} & \textbf{7.29}  & \textbf{170.50} & \textbf{1.0000} & \textbf{1.0000} \TBstrut\\ \hline
 \rowcolor{grey}
$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ2}^{N-BaIoT}$ & SN = 98.90\% , TN = 98.80\% & JSMA, $\theta$ = 0.01 & --     & --     & --      & FAIL\textsuperscript{*}   & --      \TBstrut\\ \hline

$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ2}^{N-BaIoT}$ & SN = 98.90\% , TN = 98.80\% & LBFGS, default parameter & 22.57 & 9.98  & 106.42 & 0.9960 & 0.0040 \TBstrut\\ \hline
 \rowcolor{grey}
$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ2}^{N-BaIoT}$ & SN = 98.90\% , TN = 98.80\% & PGD, default parameter & 19.59 & 19.71 & 54.00  & 1.0000 & 0.0104 \TBstrut\\ \hline

$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ2}^{N-BaIoT}$ & SN = 98.90\% , TN = 98.80\% & Deepfool, default parameter & 20.86 & 12.15 & 143.31 & 0.9190 & 0.1336 \TBstrut\\ \hline

 \rowcolor{grey}
$N_{SPRITZ2}^{N-BaIoT}$ & $N_{SPRITZ1}^{N-BaIoT}$ & SN = 98.90\% , TN = 98.80\% & I-FGSM, $\varepsilon$ = 0.1 & 17.98 & 22.67 & 58.06 & 0.9913 & 0.0200 \TBstrut\\ \hline

$N_{SPRITZ2}^{N-BaIoT}$ & $N_{SPRITZ1}^{N-BaIoT}$ & SN = 98.90\% , TN = 98.80\% & I-FGSM, $\varepsilon$ = 0.01 & 18.65 & 20.96 & 53.47 & 1.0000 & 0.0000 \TBstrut\\ \hline
 \rowcolor{grey}
$N_{SPRITZ2}^{N-BaIoT}$ & $N_{SPRITZ1}^{N-BaIoT}$ & SN = 98.90\% , TN = 98.80\% & I-FGSM, $\varepsilon$ = 0.001 & 18.71 & 20.82 & 53.16 & 1.0000 & 0.0000\TBstrut\\ \hline

$N_{SPRITZ2}^{N-BaIoT}$ & $N_{SPRITZ1}^{N-BaIoT}$ & SN = 98.90\% , TN = 98.80\% & JSMA, $\theta$ = 0.1 & 22.23 & 2.91 & 178.08 & 1.0000 & 0.0000 \TBstrut\\ \hline
 \rowcolor{grey}
$N_{SPRITZ2}^{N-BaIoT}$ & $N_{SPRITZ1}^{N-BaIoT}$ & SN = 98.90\% , TN = 98.80\% & \textbf{JSMA, $\theta$ = 0.01} &  \textbf{40.93} & \textbf{0.30} & \textbf{17.84} & \textbf{1.0000} & \textbf{0.9960} \TBstrut\\ \hline

$N_{SPRITZ2}^{N-BaIoT}$ & $N_{SPRITZ1}^{N-BaIoT}$ & SN = 98.90\% , TN = 98.80\% & LBFGS, default parameter &  24.62 & 4.67 & 114.36 & 1.0000 & 0.0000\TBstrut\\ \hline
 \rowcolor{grey}
$N_{SPRITZ2}^{N-BaIoT}$ & $N_{SPRITZ1}^{N-BaIoT}$ & SN = 98.90\% , TN = 98.80\% & PGD, default parameter & 18.75 & 20.66 & 53.07 & 1.0000 & 0.0000 \TBstrut\\ \hline

$N_{SPRITZ2}^{N-BaIoT}$ & $N_{SPRITZ1}^{N-BaIoT}$ & SN = 98.90\% , TN = 98.80\% & DeepFool, default parameter & 23.86 & 4.59 & 177.38 & 1.0000 & 0.0000 \TBstrut\\ \hline

 \rowcolor{grey}
$N_{SPRITZ1}^{DGA}$ & $N_{SPRITZ2}^{DGA}$ & SN = 99.60\% , TN = 99.60\% & I-FGSM, $\varepsilon$ = 0.1 & 31.46 & 4.81 & 17.20 & 1.0000 & 0.0100 \TBstrut\\ \hline

$N_{SPRITZ1}^{DGA}$ & $N_{SPRITZ2}^{DGA}$ & SN = 99.60\% , TN = 99.60\% & I-FGSM, $\varepsilon$ = 0.01 & 32.51 & 4.21 & 15.92 & 1.0000 & 0.0000 \TBstrut\\ \hline
 \rowcolor{grey}
$N_{SPRITZ1}^{DGA}$ & $N_{SPRITZ2}^{DGA}$ & SN = 99.60\% , TN = 99.60\% & I-FGSM, $\varepsilon$ = 0.001 &  32.96 & 4.00 & 15.03 & 1.0000 & 0.0000 \TBstrut\\ \hline

$N_{SPRITZ1}^{DGA}$ & $N_{SPRITZ2}^{DGA}$ & SN = 99.60\% , TN = 99.60\% & JSMA, $\theta$ = 0.1 & 31.23 & 1.47 & 62.50 & 1.0000 & 0.5020 \TBstrut\\ \hline
 \rowcolor{grey}
$N_{SPRITZ1}^{DGA}$ & $N_{SPRITZ2}^{DGA}$ & SN = 99.60\% , TN = 99.60\% & JSMA, $\theta$ = 0.01 & 35.95 & 1.07 & 17.85 & 1.0000 & 0.0900 \TBstrut\\ \hline

$N_{SPRITZ1}^{DGA}$ & $N_{SPRITZ2}^{DGA}$ & SN = 99.60\% , TN = 99.60\% & LBFGS, default parameter & 37.19 & 1.47  & 23.20 & 0.9930 & 0.0400 \TBstrut\\ \hline
 \rowcolor{grey}
$N_{SPRITZ1}^{DGA}$ & $N_{SPRITZ2}^{DGA}$ & SN = 99.60\% , TN = 99.60\% & PGD, default parameter & 33.75 & 3.58 & 13.93 & 1.0000 & 0.0000 \TBstrut\\ \hline

$N_{SPRITZ1}^{DGA}$ & $N_{SPRITZ2}^{DGA}$ & SN = 99.60\% , TN = 99.60\% & DeepFool, default parameter & 34.11 & 2.20 & 38.21 & 1.0000 & 0.0000 \TBstrut\\ \hline

 \rowcolor{grey}
$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ1}^{DGA}$ & SN = 99.60\% , TN = 99.60\% & I-FGSM, $\varepsilon$ = 0.1 &  28.48 & 6.04 & 24.15 & 1.0000 & 0.4100 \TBstrut\\ \hline

$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ1}^{DGA}$ & SN = 99.60\% , TN = 99.60\% & \textbf{I-FGSM, $\varepsilon$ = 0.01} & \textbf{28.62} & \textbf{5.99} & \textbf{23.25} & \textbf{1.0000} & \textbf{1.0000} \TBstrut\\ \hline
 \rowcolor{grey}
$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ1}^{DGA}$ & SN = 99.60\% , TN = 99.60\% & \textbf{I-FGSM, $\varepsilon$ = 0.001} & \textbf{28.92} & \textbf{5.76} & \textbf{22.64} & \textbf{1.0000} & \textbf{1.0000} \TBstrut\\ \hline

$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ1}^{DGA}$ & SN = 99.60\% , TN = 99.60\% & JSMA, $\theta$ = 0.1 & 31.17 & 1.28 & 56.56 & 1.0000 & 0.0000  \TBstrut\\ \hline
 \rowcolor{grey}
$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ1}^{DGA}$ & SN = 99.60\% , TN = 99.60\% & JSMA, $\theta$ = 0.01 & --     & --     & --      & FAIL\textsuperscript{*}   & --  \TBstrut\\ \hline

$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ1}^{DGA}$ & SN = 99.60\% , TN = 99.60\% & \textbf{LBFGS, default parameter} &  \textbf{34.22} & \textbf{1.48} & \textbf{33.92} & \textbf{0.9930} & \textbf{0.6300} \TBstrut\\ \hline
 \rowcolor{grey}
$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ1}^{DGA}$ & SN = 99.60\% , TN = 99.60\% & PGD, default parameter & 29.24 & 5.49 & 22.24 & 1.0000 & 0.3200  \TBstrut\\ \hline

$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ1}^{DGA}$ & SN = 99.60\% , TN = 99.60\% & DeepFool, default parameter & 31.02 & 2.25 & 53.42 & 1.0000 & 0.2329   \TBstrut\\ \hline

\rowcolor{grey}
$N_{SPRITZ1}^{RIPE}$ & $N_{SPRITZ2}^{RIPE}$ & SN = 98.90\% , TN = 99.80\% & I-FGSM, $\varepsilon$ = 0.1 & 18.65 & 22.07 & 64.78  & 1.0000 & 0.0000 \TBstrut\\ \hline

$N_{SPRITZ1}^{RIPE}$ & $N_{SPRITZ2}^{RIPE}$ & SN = 98.90\% , TN = 99.80\% & \textbf{JSMA, $\theta$ = 0.1} & \textbf{18.49} & \textbf{7.29}  & \textbf{170.50} & \textbf{1.0000} & \textbf{0.0140} \TBstrut\\ \hline

\rowcolor{grey}
$N_{SPRITZ1}^{RIPE}$ & $N_{SPRITZ2}^{RIPE}$ & SN = 98.90\% , TN = 99.80\% & LBFGS, default parameter & 22.57 & 9.98  & 106.42 & 0.9960 & 0.0100 \TBstrut\\ \hline


$N_{SPRITZ1}^{RIPE}$ & $N_{SPRITZ2}^{RIPE}$ & SN = 99.60\% , TN = 99.80\% & PGD, default parameter & 33.75 & 3.58 & 13.93 & 1.0000 & 0.0020 \TBstrut\\ \hline

\rowcolor{grey}
$N_{SPRITZ1}^{RIPE}$ & $N_{SPRITZ2}^{RIPE}$ & SN = 99.60\% , TN = 99.80\% & DeepFool, default parameter & 34.11 & 2.20 & 38.21 & 1.0000 & 0.0000 \TBstrut\\ \hline

\end{tabular}}
\\FAIL\textsuperscript{*}: In this case, the attack on the source network fails and we cannot transfer it to the target network. Therefore, the numerical values of the average PSNR, the average $L_1$ dist, and the average maximum distortion are not possible.  
\end{table*}

==> Tables/CrossModelTraining/CMT.tex <==
\begin{table*}[!h]
%\scriptsize
\centering
\caption{Experimental results for Cross Model and Training Transferability\\. \label{CMT}}
\resizebox{2\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{SN} & \textbf{TN} & \textbf{Accuracy} & \textbf{Attack Type} & \textbf{PSNR} & \textbf{$L_1$ dist} & \textbf{Max. dist} & \textbf{ASR} & \textbf{ASR} \TBstrut\\
& & & & & & & \textbf{(SN)} & \textbf{(TN)}  \\ \hline
 \rowcolor{grey}
$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ2}^{DGA}$ & SN = 98.80\% , TN = 100\% & I-FGSM, $\varepsilon$ = 0.1 & 18.65 & 22.07 & 64.78  & 1.0000 & 0.0030 \TBstrut\\ \hline

$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ2}^{DGA}$ & SN = 98.80\% , TN = 100\% & I-FGSM, $\varepsilon$ = 0.01 & 18.93 & 21.26 & 62.71  & 1.0000 & 0.0000 \TBstrut\\ \hline
 \rowcolor{grey}
$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ2}^{DGA}$ & SN = 98.80\% , TN = 100\% & I-FGSM, $\varepsilon$ = 0.001 & 19.06 & 20.93 & 61.72  & 1.0000 & 0.0000 \TBstrut\\ \hline

$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ2}^{DGA}$ & SN = 98.80\% , TN = 100\% & JSMA, $\theta$ = 0.1 & 18.49 & 7.29  & 178.50 & 1.0000 & 0.0000 \TBstrut\\ \hline
 \rowcolor{grey}
$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ2}^{DGA}$ & SN = 98.80\% , TN = 100\% & JSMA, $\theta$ = 0.01 & --     & --     & --      & FAIL\textsuperscript{*}   & --      \TBstrut\\ \hline

$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ2}^{DGA}$ & SN = 98.80\% , TN = 100\% & LBFGS, default parameter & 22.57 & 10.46 & 110.67 & 0.9910 & 0.0000 \TBstrut\\ \hline
 \rowcolor{grey}
$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ2}^{DGA}$ & SN = 98.80\% , TN = 100\% & PGD, default parameter & 19.59 & 19.71 & 54.00  & 1.0000 & 0.0000 \TBstrut\\ \hline

$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ2}^{DGA}$ & SN = 98.80\% , TN = 100\% & DeepFool, default parameter & 20.87 & 12.14 & 143.19 & 0.9676 & 0.0324 \TBstrut\\ \hline

 \rowcolor{grey}
$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ1}^{N-BaIoT}$ & SN = 99.60\% , TN = 99.60\% & I-FGSM, $\varepsilon$ = 0.1 & 28.49 & 6.03 & 24.15 & 1.0000 & 0.0400 \TBstrut\\ \hline

$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ1}^{N-BaIoT}$ & SN = 99.60\% , TN = 99.60\% & I-FGSM, $\varepsilon$ = 0.01 & 28.62 & 5.99 & 23.25 & 1.0000 & 0.0000 \TBstrut\\ \hline
 \rowcolor{grey}
$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ1}^{N-BaIoT}$ & SN = 99.60\% , TN = 99.60\% & I-FGSM, $\varepsilon$ = 0.001 & 28.92 & 5.76 & 22.64 & 1.0000 & 0.0000 \TBstrut\\ \hline

$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ1}^{N-BaIoT}$ & SN = 99.60\% , TN = 99.60\% & JSMA, $\theta$ = 0.1 & 31.17 & 1.28 & 56.56 & 1.0000 & 0.0000  \TBstrut\\ \hline
 \rowcolor{grey}
$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ1}^{N-BaIoT}$ & SN = 99.60\% , TN = 99.60\% & JSMA, $\theta$ = 0.01 & --     & --    & --     & FAIL\textsuperscript{*}   & --      \TBstrut\\ \hline

$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ1}^{N-BaIoT}$ & SN = 99.60\% , TN = 99.60\% & LBFGS, default parameter & 34.22 & 1.40 & 33.93 & 0.9860 & 0.0040 \TBstrut\\ \hline
 \rowcolor{grey}
$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ1}^{N-BaIoT}$ & SN = 99.60\% , TN = 99.60\% & PGD, default parameter & 29.24 & 5.99 & 22.24 & 1.0000 & 0.0000 \TBstrut\\ \hline

$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ1}^{N-BaIoT}$ & SN = 99.60\% , TN = 99.60\% & DeepFool, default parameter & 31.02 & 2.59 & 53.42 & 1.0000 & 0.0104 \TBstrut\\ \hline

 \rowcolor{grey}
$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ2}^{RIPE}$ & SN = 98.80\% , TN = 99.80\% & I-FGSM, $\varepsilon$ = 0.1 & 18.65 & 22.07 & 64.78  & 1.0000 & 0.0000 \TBstrut\\ \hline

$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ2}^{RIPE}$ & SN = 98.80\% , TN = 99.80\% & JSMA, $\theta$ = 0.1 & 18.49 & 7.29  & 178.50 & 1.0000 & 0.0010 \TBstrut\\ \hline

 \rowcolor{grey}
$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ2}^{RIPE}$ & SN = 98.80\% , TN = 99.80\% & LBFGS, default parameter & 22.57 & 10.46 & 110.67 & 0.9910 & 0.0000 \TBstrut\\ \hline


$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ2}^{RIPE}$ & SN = 98.80\% , TN = 99.80\% & PGD, default parameter & 19.59 & 19.71 & 54.00  & 1.0000 & 0.0000 \TBstrut\\ \hline

\rowcolor{grey}
$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ2}^{RIPE}$ & SN = 98.80\% , TN = 99.80\% & DeepFool, default parameter & 20.87 & 12.14 & 143.19 & 0.9676 & 0.0200 \TBstrut\\ \hline

\end{tabular}}
\\FAIL\textsuperscript{*}: In this case, the attack on the source network fails and we cannot transfer it to the target network. Therefore, the numerical values of the average PSNR, the average $L_1$ dist, and the average maximum distortion are not possible. 
\end{table*}












==> Tables/CrossTraining/CT_SPRITZ1_First.tex <==
\begin{table*}[!h]
%\scriptsize
\centering
\caption{Experimental Results for Cross Training Transferability on SPRITZ1 and SPRITZ2 Architecture\\ (N-BaIoT and DGA datasets are used interchangeably in the SN and the TN). \label{CT_SPRITZ1_First}}
\resizebox{2\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{SN} & \textbf{TN} & \textbf{Accuracy} & \textbf{Attack Type} & \textbf{PSNR} & \textbf{$L_1$ dist} & \textbf{Max. dist} & \textbf{ASR} & \textbf{ASR} \TBstrut\\
& & & & & & & \textbf{(SN)} & \textbf{(TN)}  \\ \hline
 \rowcolor{grey}
$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ1}^{DGA}$ & SN = 98.90\% , TN = 100\% & I-FGSM, $\varepsilon$ = 0.1 & 18.65 & 22.07 & 65.12 & 1.0000 & 0.0480 \TBstrut\\ \hline

$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ1}^{DGA}$ & SN = 98.90\% , TN = 100\% & I-FGSM, $\varepsilon$ = 0.01 & 18.93 & 21.26 & 62.71 & 1.0000 & 0.0000 \TBstrut\\ \hline
 \rowcolor{grey}
$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ1}^{DGA}$ & SN = 98.90\% , TN = 100\% & I-FGSM, $\varepsilon$ = 0.001 & 19.06 & 20.94 & 61.76 & 1.0000 & 0.0000 \TBstrut\\ \hline

$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ1}^{DGA}$ & SN = 98.90\% , TN = 100\% & JSMA, $\theta$ = 0.1 & 18.49 & 7.29 & 178.50 & 1.0000 & 0.1100 \TBstrut\\ \hline
 \rowcolor{grey}
$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ1}^{DGA}$ & SN = 98.90\% , TN = 100\% & JSMA, $\theta$ = 0.01 & -- & -- & -- & FAIL\textsuperscript{*} & -- \TBstrut\\ \hline

$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ1}^{DGA}$ & SN = 98.90\% , TN = 100\% & LBFGS, default parameter & 22.57 & 9.98 & 106.35 & 1.0000 & 0.0000 \TBstrut\\ \hline
 \rowcolor{grey}
$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ1}^{DGA}$ & SN = 98.90\% , TN = 100\% & PGD, default parameter & 19.59 & 19.71 & 54.00 & 0.9800 & 0.0020 \TBstrut\\ \hline

$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ1}^{DGA}$ & SN = 98.90\% , TN = 100\% & DeepFool, default parameter & 20.90 & 12.11 & 142.85 & 0.9500 & 0.0400 \TBstrut\\ \hline


 \rowcolor{grey}
$N_{SPRITZ1}^{DGA}$ & $N_{SPRITZ1}^{N-BaIoT}$ & SN = 100\% , TN = 98.90\% & I-FGSM, $\varepsilon$ = 0.1 & 31.4618 & 4.81 & 17.20 & 1.0000 & 0.0050 \TBstrut\\ \hline

$N_{SPRITZ1}^{DGA}$ & $N_{SPRITZ1}^{N-BaIoT}$ & SN = 100\% , TN = 98.90\% & I-FGSM, $\varepsilon$ = 0.01 & 32.51 & 4.21 & 15.92 & 1.0000 & 0.0000 \TBstrut\\ \hline
 \rowcolor{grey}
$N_{SPRITZ1}^{DGA}$ & $N_{SPRITZ1}^{N-BaIoT}$ & SN = 100\% , TN = 98.90\% & I-FGSM, $\varepsilon$ = 0.001 & 32.96 & 4.00 & 15.03 & 1.0000 & 0.0000 \TBstrut\\ \hline

$N_{SPRITZ1}^{DGA}$ & $N_{SPRITZ1}^{N-BaIoT}$ & SN = 100\% , TN = 98.90\% & JSMA, $\theta$ = 0.1 & 31.23 & 1.47 & 62.50 & 1.0000 & 0.2000 \TBstrut\\ \hline
 \rowcolor{grey}
$N_{SPRITZ1}^{DGA}$ & $N_{SPRITZ1}^{N-BaIoT}$ & SN = 100\% , TN = 98.90\% & JSMA, $\theta$ = 0.01 & 35.95 & 1.077 & 17.85 & 1.0000 & 0.0010 \TBstrut\\ \hline

$N_{SPRITZ1}^{DGA}$ & $N_{SPRITZ1}^{N-BaIoT}$ & SN = 100\% , TN = 98.90\% & LBFGS, default parameter & 37.19 & 1.41 & 23.38 & 1.0000 & 0.0000 \TBstrut\\ \hline
 \rowcolor{grey}
$N_{SPRITZ1}^{DGA}$ & $N_{SPRITZ1}^{N-BaIoT}$ & SN = 100\% , TN = 98.90\% & PGD, default parameter &  33.75 & 3.58 & 13.93 & 1.0000 & 0.0000\TBstrut\\ \hline

$N_{SPRITZ1}^{DGA}$ & $N_{SPRITZ1}^{N-BaIoT}$ & SN = 100\% , TN = 98.90\% & DeepFool, default parameter &  36.98 & 2.20 & 38.08 & 1.0000 & 0.0300 \TBstrut\\ \hline

 \rowcolor{grey}
$N_{SPRITZ2}^{N-BaIoT}$ & $N_{SPRITZ2}^{DGA}$ & SN = 98.90\% , TN = 100\% & I-FGSM, $\varepsilon$ = 0.1 & 17.98 & 22.67 & 58.06  & 1.0000 & 0.0360  \TBstrut\\ \hline

$N_{SPRITZ2}^{N-BaIoT}$ & $N_{SPRITZ2}^{DGA}$ & SN = 98.90\% , TN = 100\% & I-FGSM, $\varepsilon$ = 0.01 & 18.64 & 20.96 & 53.47  & 1.0000 & 0.0000 \TBstrut\\ \hline
 \rowcolor{grey}
$N_{SPRITZ2}^{N-BaIoT}$ & $N_{SPRITZ2}^{DGA}$ & SN = 98.90\% , TN = 100\% & I-FGSM, $\varepsilon$ = 0.001 & 18.71 & 20.82 & 53.16  & 1.0000 & 0.0000 \TBstrut\\ \hline

$N_{SPRITZ2}^{N-BaIoT}$ & $N_{SPRITZ2}^{DGA}$ & SN = 98.90\% , TN = 100\% & JSMA, $\theta$ = 0.1 & 22.23 & 2.91  & 178.08 & 1.0000 & 0.0061 \TBstrut\\ \hline
 \rowcolor{grey}
$N_{SPRITZ2}^{N-BaIoT}$ & $N_{SPRITZ2}^{DGA}$ & SN = 98.90\% , TN = 100\% & JSMA, $\theta$ = 0.01 & -- & -- & -- & FAIL\textsuperscript{*} & -- \TBstrut\\ \hline

$N_{SPRITZ2}^{N-BaIoT}$ & $N_{SPRITZ2}^{DGA}$ & SN = 98.90\% , TN = 100\% & LBFGS, default parameter & 24.62 & 4.67  & 194.25 & 1.0000 & 0.0000 \TBstrut\\ \hline
 \rowcolor{grey}
$N_{SPRITZ2}^{N-BaIoT}$ & $N_{SPRITZ2}^{DGA}$ & SN = 98.90\% , TN = 100\% & PGD, default parameter & 18.75 & 20.66 & 53.07  & 0.9916 & 0.1812 \TBstrut\\ \hline

$N_{SPRITZ2}^{N-BaIoT}$ & $N_{SPRITZ2}^{DGA}$ & SN = 98.90\% , TN = 100\% & DeepFool, default parameter & 23.86 & 4.59  & 177.38 & 1.0000 & 0.0000 \TBstrut\\ \hline
 \rowcolor{grey}
$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ2}^{N-BaIoT}$ & SN = 100\% , TN = 98.90\% & I-FGSM, $\varepsilon$ = 0.1 & 28.48 & 6.03 & 25.15 & 0.9800 & 0.0150\TBstrut\\ \hline

$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ2}^{N-BaIoT}$ & SN = 100\% , TN = 98.90\% & I-FGSM, $\varepsilon$ = 0.01 &  28.61 & 5.99 & 23.34 & 1.0000 & 0.0000 \TBstrut\\ \hline
 \rowcolor{grey}
$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ2}^{N-BaIoT}$ & SN = 100\% , TN = 98.90\% & I-FGSM, $\varepsilon$ = 0.001 &  28.92 & 5.76 & 22.64 & 1.0000 & 0.0000\TBstrut\\ \hline

$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ2}^{N-BaIoT}$ & SN = 100\% , TN = 98.90\% & JSMA, $\theta$ = 0.1 & 31.17 & 1.28 & 56.56 & 1.0000 & 0.1000 \TBstrut\\ \hline
 \rowcolor{grey}
$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ2}^{N-BaIoT}$ & SN = 100\% , TN = 98.90\% & JSMA, $\theta$ = 0.01 & -- & -- & -- & FAIL\textsuperscript{*} & -- \TBstrut\\ \hline

$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ2}^{N-BaIoT}$ & SN = 100\% , TN = 98.90\% & LBFGS, default parameter & 34.22 & 1.40 & 33.93 & 1.0000 & 0.0000 \TBstrut\\ \hline
 \rowcolor{grey}
$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ2}^{N-BaIoT}$ & SN = 100\% , TN = 98.90\% & PGD, default parameter & 29.24 & 5.49 & 22.24 & 1.0000 & 0.0000 \TBstrut\\ \hline

$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ2}^{N-BaIoT}$ & SN = 100\% , TN = 98.90\% & DeepFool, default parameter & 31.02 & 2.25 & 53.42 & 0.9812 & 0.1200  \TBstrut\\ \hline

 \rowcolor{grey}
$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ1}^{RIPE}$ & SN = 98.90\% , TN = 99.20\% & I-FGSM, $\varepsilon$ = 0.1 & 18.65 & 22.07 & 65.12 & 1.0000 & 0.0200 \TBstrut\\ \hline

$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ1}^{RIPE}$ & SN = 98.90\% , TN = 99.20\% & JSMA, $\theta$ = 0.1 & 18.49 & 7.29 & 178.50 & 1.0000 & 0.0000 \TBstrut\\ \hline

$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ1}^{RIPE}$ & SN = 98.90\% , TN = 99.20\% & LBFGS, default parameter & 22.57 & 9.98 & 106.35 & 1.0000 & 0.0010 \TBstrut\\ \hline

 \rowcolor{grey}
$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ1}^{RIPE}$ & SN = 98.90\% , TN = 99.20\% & PGD, default parameter & 19.59 & 19.71 & 54.00 & 0.9800 & 0.0000 \TBstrut\\ \hline

$N_{SPRITZ1}^{DGA}$ & $N_{SPRITZ1}^{RIPE}$ & SN = 98.90\% , TN = 99.20\% & DeepFool, default parameter &  36.98 & 2.20 & 38.08 & 1.0000 & 0.0000 \TBstrut\\ \hline

\end{tabular}}
\\FAIL\textsuperscript{*}: In this case, the attack on the source network fails and we cannot transfer it to the target network. Therefore, the numerical values of the average PSNR, the average $L_1$ dist, and the average maximum distortion are not possible.  
\end{table*}

==> Tables/DefenseMPA.tex <==
\begin{table*}[!h]
%\scriptsize
\centering
\caption{\violet{Test Accuracy Values TN with an MPA fine-tunning.} \label{Defense_MPA}}
\begin{tabular}{@{}|>{\color{violet}}c |>{\color{violet}}c |>{\color{violet}}c |>{\color{violet}}c |>{\color{violet}}c |>{\color{violet}}c | >{\color{violet}}c |}
\hline
\textbf{TN} & \textbf{Fine-Tune} & \textbf{Parameter} & \textbf{I-FGSM, $\varepsilon$ = 0.01} & \textbf{IFGSM, $\varepsilon$ = 0.001} &\textbf{LBFGS, Default} &\textbf{JSMA, $\theta$ = 0.01}\TBstrut\\
 \hline
 \rowcolor{grey}
 
$N_{SPRITZ1}^{N-BaIoT}$ & JSMA & $\theta$ = 0.01 & 0.0000 & 0.0100 & 0.2010 & ---\TBstrut\\ \hline

$N_{SPRITZ1}^{DGA}$ & I-FGSM& $\varepsilon$ = 0.01 & --- & 0.0000 & 0.0010 & 0.0000\TBstrut\\ \hline
 \rowcolor{grey}

$N_{SPRITZ1}^{DGA}$ & I-FGSM& $\varepsilon$ = 0.001 & 0.0000 & --- & 0.0010 & 0.0000\TBstrut\\ \hline

$N_{SPRITZ1}^{DGA}$ & LBFGS& Default & 0.0200 & 0.0010 & --- & 0.0000\TBstrut\\ \hline

%SPRITZ1 & I-FGSM, $\varepsilon$ = 0.01 & N-BaIoT & DGA& 20.49 &21.57\TBstrut\\ %\hline
 %\rowcolor{grey}
%SPRITZ1 & I-FGSM, $\varepsilon$ = 0.001 & N-BaIoT &DGA& 203.98 & 212.77\TBstrut\\ %\hline

%SPRITZ1 & JSMA, $\theta$ = 0.1 & N-BaIoT &DGA& 30.41 & 10.42\TBstrut\\ \hline
 %\rowcolor{grey}
%SPRITZ1 & LBFGS, default parameter & N-BaIoT &DGA& 48.73 & 25.92\TBstrut\\ \hline

%SPRITZ1 & PGD, default parameter & N-BaIoT &DGA& 16.92 & 16.17\TBstrut\\ \hline
 %\rowcolor{grey}
%SPRITZ1 & DeepFool, default parameter & N-BaIoT &DGA& 0.49 &0.23\TBstrut\\ \hline
%

%SPRITZ2 & I-FGSM, $\varepsilon$ = 0.1 & N-BaIoT & DGA& 4.42& 4.49\TBstrut\\ \hline
%\rowcolor{grey}
%SPRITZ2 & I-FGSM, $\varepsilon$ = 0.01 & N-BaIoT & DGA& 43.94 &44.98\TBstrut\\ %\hline
 
%SPRITZ2 & I-FGSM, $\varepsilon$ = 0.001 & N-BaIoT &DGA& 438.436 & 446.969\TBstrut\\ \hline
%\rowcolor{grey}
%SPRITZ2 & JSMA, $\theta$ = 0.1 & N-BaIoT &DGA& 32.58 & 20.53\TBstrut\\ \hline
 
%SPRITZ2 & LBFGS, default parameter & N-BaIoT &DGA& 78.73 & 51.93\TBstrut\\ \hline
%\rowcolor{grey}
%SPRITZ2 & PGD, default parameter & N-BaIoT &DGA& 45.25 & 33.60\TBstrut\\ \hline
 
%SPRITZ2 & DeepFool, default parameter & N-BaIoT &DGA& 0.31 &0.37\TBstrut\\ \hline 
%$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ2}^{N-BaIoT}$ & SN = 98.90\% , TN = 98.80\% & JSMA, $\theta$ = 0.1 & 18.49 & 7.29 & 170.50 & 1.0000 & 1.0000 \TBstrut\\ \hline

%$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ1}^{DGA}$ & SN = 99.60\% , TN = 99.60\% & I-FGSM, $\varepsilon$ = 0.01 & 28.62 & 5.99 & 23.25 & 1.0000 & 1.0000 \TBstrut\\ \hline
% \rowcolor{grey}
%$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ1}^{DGA}$ & SN = 99.60\% , TN = 99.60\% & I-FGSM, $\varepsilon$ = 0.001 & 28.92 & 5.76 & 22.64 & 1.0000 & 1.0000 \TBstrut\\ \hline

%$N_{SPRITZ2}^{N-BaIoT}$ & $N_{SPRITZ1}^{N-BaIoT}$ & SN = 98.90\% , TN = 98.80\% & JSMA, $\theta$ = 0.01 & 40.93 & 0.30 & 17.84 & 1.0000 & 0.9960 \TBstrut\\ \hline
 %\rowcolor{grey}
%$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ1}^{DGA}$ & SN = 99.60\% , TN = 99.60\% & LBFGS, default parameter &  34.22 & 1.48 & 33.92 & 0.9930 & 0.6300 \TBstrut\\ \hline

\end{tabular}
\end{table*}


==> Tables/Differences.tex <==
\begin{table*}[!h]
\centering
\small
\caption{Difference between our work and existing works in 1C classifier} \label{difference}
%\begin{tabular}{|l|l|l|l|l|l|l|}
\resizebox{1\textwidth}{!}{
\begin{tabular}{|l |l |l |l |l |l | l |}
\hline
\textbf{Ref.} & \textbf{Application Domain} & \textbf{Classifier} & \textbf{Considered Datasets} & \textbf{Advantages} & \textbf{Disadvantages} & \textbf{Year}   \\ \hline

    \cite{perdisci2006using} & Anomaly IDS & -One-Class SVM          &      -Private Dataset & -ADV & -DISADV & 2006                         \\ \hline
    
    \cite{scheirer2012toward} & Face Verification & -One-Class SVM          &      -Caltech and -ImageNet & -ADV & -DISADV & 2013                         \\ \hline


    \cite{marchi2015novel} & Acoustic novelty detection & -LSTM and -Autoencoder          &      -PASCAL CHiME & -Denoising and -Good Performance & -dataset is not for real events & 2015                         \\ \hline
   
  
    \cite{d2017autoencoder} & Video forgery detection & -LSTM and -Autoencoder          &      -GRIP & ADV & DISADV & 2017                         \\ \hline
    
    \cite{henrydoss2017incremental} & incremental open set intrusion detection & -EVM         &      -KDDCUP’99 & supports incremental learning & \makecell[l]{-high soft-margin errors \\ -Not optimized EVM algorithm} & 2017                         \\ \hline
    
    \cite{9053318} & \makecell[l]{attack transferability between \\ deep learning networks} & -CNN and -SVM          &      -RAISE & ADV & DISADV & 2020                         \\ \hline
    
    \cite{MOTI2021102591} & detect unseen Internet of Things malware & -CNN, -GAN and -LSTM          &      \makecell[l]{-Windows and IoT \\ malware datasets} & \makecell[l]{-higher detection rate \\ -can be used in settings with \\insufficient or imbalanced data}  & DISADV & 2021                         \\ \hline
   
   \cite{xu2022improved} & Network Intrusion Detection & -Bi-GAN          &      \makecell[l]{-NSL-KDD \\ -CIC-DDoS2019} & less training overhead & DISADV & 2022                         \\ \hline
   
   \cite{huang2022novel} &  open set authentication of IoT  & -CNN and -OpenMAX          &      -ADS–B & Applicable on real world problems & low robustness of the features & 2022                         \\ \hline
   
   \cite{sawadogo2022android} &  android malware detection  & -13 different classifiers  &      -Private Dataset & ADV & DISADV & 2022                         \\ \hline
   
   \cite{akgun2022new} &  DDoS attacks intrusion detection  & -DNN, -CNN and -LSTM  &      -CIC-DDoS2019 & \makecell[l]{-Good inference time \\ -smaller number of trainable parameters}  & DISADV & 2022                         \\ \hline
   
   \cite{9747933} &  computer networks security  & -CNN  &      \makecell[l]{-N-BaIoT \\ -DGA \\ -RIPE Atlas} & -ADV  & -responds to a few adversarial attacks & 2022                         \\ \hline
\end{tabular}}
\end{table*}

==> Tables/Networks.tex <==
\begin{table}[!h]
%\scriptsize
\centering
\caption{General Description of the Considered Networks with their Respective Datasets. \label{Networks}}
\begin{tabular}{|c|c|c|c|}
\hline
\backslashbox{Networks}{Datasets} & \textbf{N-BaIoT} & \textbf{DGA}& \textbf{RIPE}\TBstrut\\ \hline

\textbf{SPRITZ1} & $N_{SPRITZ1}^{N-BaIoT}$ &  $N_{SPRITZ1}^{DGA}$ & $N_{SPRITZ1}^{RIPE}$\TBstrut\\\hline

\textbf{SPRITZ2} & $N_{SPRITZ2}^{N-BaIoT}$ & $N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ2}^{RIPE}$\TBstrut\\\hline

\end{tabular}
\end{table}

==> Tables/RelatedWorks/RelatedWorks.tex <==
\begin{table}[!h]
%\scriptsize
%\footnotesize
\centering
\small
\caption{Acronyms and Abbreviations List. \label{Abbreviations}}
\begin{tabular}{@{}|c|l|}
\hline
\textbf{Acronym} & \textbf{Description} \\ \hline

CNN & Convolutional Neural Network \\ \hline

FR & Feature Randomization \\ \hline

LK & Limited Knowledge \\ \hline

SK & Semi Limited Knowledge \\ \hline

PK & Perfect Knowledge \\ \hline

SVM & Support Vector Machine \\ \hline

ML & Machine Learning \\ \hline

DL & Deep Learning \\ \hline

SN & Source Network\\ \hline

TN & Target Network\\ \hline

$N_1$, $N_2$ & Shallow Network, Deep Network \\ \hline

ASR & Attack Success Rate \\ \hline

Max. dist & Maximum distortion\\ \hline

PSNR & Peak signal-to-noise ratio\\ \hline

$L_1$ dist & $L_1$ distance\\ \hline

I-FGSM & Iterative-Fast Gradient Sign Method \\ \hline

PGD  & Projected Gradient Descent\\ \hline

JSMA  & Jacobian Saliency Map Attack\\ \hline

BIM & Basic Iterative Method \\ \hline

C\&W & Carlini \& Wagner \\ \hline

L-BFGS  &  Limited-memory Broyden-Fletcher-Goldfarb-Shanno\\ \hline

FGSM & Fast Gradient Sign Method\\ \hline

MPA & Most Powerful Attacks \\ \hline

Lr & learning rate \\ \hline
\end{tabular}
\end{table}






==> Tables/Transferability.tex <==
\begin{table*}[!h]
%\scriptsize
\centering
\caption{Summary of Transferability cases. \label{Transferability}}
\begin{tabular}{@{}|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{SN} & \textbf{TN} & \textbf{Accuracy} & \textbf{Attack Type} & \textbf{PSNR} & \textbf{$L_1$ dist} & \textbf{Max. dist} & \textbf{ASR} & \textbf{ASR} \TBstrut\\
& & & & & & & \textbf{(SN)} & \textbf{(TN)}  \\ \hline
 \rowcolor{grey}
$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ2}^{N-BaIoT}$ & SN = 98.90\% , TN = 98.80\% & JSMA, $\theta$ = 0.1 & 18.49 & 7.29 & 170.50 & 1.0000 & 1.0000 \TBstrut\\ \hline

$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ1}^{DGA}$ & SN = 99.60\% , TN = 99.60\% & I-FGSM, $\varepsilon$ = 0.01 & 28.62 & 5.99 & 23.25 & 1.0000 & 1.0000 \TBstrut\\ \hline
 \rowcolor{grey}
$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ1}^{DGA}$ & SN = 99.60\% , TN = 99.60\% & I-FGSM, $\varepsilon$ = 0.001 & 28.92 & 5.76 & 22.64 & 1.0000 & 1.0000 \TBstrut\\ \hline

$N_{SPRITZ2}^{N-BaIoT}$ & $N_{SPRITZ1}^{N-BaIoT}$ & SN = 98.90\% , TN = 98.80\% & JSMA, $\theta$ = 0.01 & 40.93 & 0.30 & 17.84 & 1.0000 & 0.9960 \TBstrut\\ \hline
 \rowcolor{grey}
$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ1}^{DGA}$ & SN = 99.60\% , TN = 99.60\% & LBFGS, default parameter &  34.22 & 1.48 & 33.92 & 0.9930 & 0.6300 \TBstrut\\ \hline

\end{tabular}
\end{table*}

==> Tables/executionTime.tex <==
\begin{table*}[!th]
%\scriptsize
\centering
\caption{\red{Execution running attack time on SN.} \label{Exe_Time}}
\resizebox{2\columnwidth}{!}{
\begin{tabular}{@{}|>{\color{red}}c |>{\color{red}}c |>{\color{red}}c |>{\color{red}}c |>{\color{red}}c |>{\color{red}}c |>{\color{red}}c |>{\color{red}}c|}
\hline
\textbf{SN} & \textbf{Attack Type} & \textbf{Dataset1} & \textbf{Dataset2} & \textbf{Dataset3}& \textbf{Exe. min (Dataset1)} &\textbf{Exe. min (Dataset2)} &\textbf{Exe. min (Dataset3)}\TBstrut\\
 \hline
 \rowcolor{grey}
 
SPRITZ1 & I-FGSM, $\varepsilon$ = 0.1 & N-BaIoT & DGA&RIPE &2.12& 2.13&2.18\TBstrut\\ \hline

SPRITZ1 & I-FGSM, $\varepsilon$ = 0.01 & N-BaIoT & DGA&RIPE & 20.49 &21.57& ---\TBstrut\\ \hline
 \rowcolor{grey}
SPRITZ1 & I-FGSM, $\varepsilon$ = 0.001 & N-BaIoT &DGA&RIPE & 203.98 & 212.77& ---\TBstrut\\ \hline

SPRITZ1 & JSMA, $\theta$ = 0.1 & N-BaIoT &DGA&RIPE & 30.41 & 10.42&30.67\TBstrut\\ \hline
 \rowcolor{grey}
SPRITZ1 & LBFGS, default parameter & N-BaIoT &DGA&RIPE & 48.73 & 25.92& 40.92\TBstrut\\ \hline

SPRITZ1 & PGD, default parameter & N-BaIoT &DGA&RIPE & 16.92 & 16.17, &16.27\TBstrut\\ \hline
 \rowcolor{grey}
SPRITZ1 & DeepFool, default parameter & N-BaIoT &DGA&RIPE &0.49 &0.23&0.38\TBstrut\\ \hline
%

SPRITZ2 & I-FGSM, $\varepsilon$ = 0.1 & N-BaIoT & DGA& RIPE &4.42& 4.49& ---\TBstrut\\ \hline
\rowcolor{grey}
SPRITZ2 & I-FGSM, $\varepsilon$ = 0.01 & N-BaIoT & DGA&RIPE & 43.94 &44.98& ---\TBstrut\\ \hline
 
SPRITZ2 & I-FGSM, $\varepsilon$ = 0.001 & N-BaIoT &DGA&RIPE & 438.436 & 446.969& ---\TBstrut\\ \hline
\rowcolor{grey}
SPRITZ2 & JSMA, $\theta$ = 0.1 & N-BaIoT &DGA&RIPE & 32.58 & 20.53& ---\TBstrut\\ \hline
 
SPRITZ2 & LBFGS, default parameter & N-BaIoT &DGA&RIPE & 78.73 & 51.93& ---\TBstrut\\ \hline
\rowcolor{grey}
SPRITZ2 & PGD, default parameter & N-BaIoT &DGA&RIPE & 45.25 & 33.60& ---\TBstrut\\ \hline
 
SPRITZ2 & DeepFool, default parameter & N-BaIoT &DGA&RIPE & 0.31 &0.37 & ---\TBstrut\\ \hline 
%$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ2}^{N-BaIoT}$ & SN = 98.90\% , TN = 98.80\% & JSMA, $\theta$ = 0.1 & 18.49 & 7.29 & 170.50 & 1.0000 & 1.0000 \TBstrut\\ \hline

%$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ1}^{DGA}$ & SN = 99.60\% , TN = 99.60\% & I-FGSM, $\varepsilon$ = 0.01 & 28.62 & 5.99 & 23.25 & 1.0000 & 1.0000 \TBstrut\\ \hline
% \rowcolor{grey}
%$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ1}^{DGA}$ & SN = 99.60\% , TN = 99.60\% & I-FGSM, $\varepsilon$ = 0.001 & 28.92 & 5.76 & 22.64 & 1.0000 & 1.0000 \TBstrut\\ \hline

%$N_{SPRITZ2}^{N-BaIoT}$ & $N_{SPRITZ1}^{N-BaIoT}$ & SN = 98.90\% , TN = 98.80\% & JSMA, $\theta$ = 0.01 & 40.93 & 0.30 & 17.84 & 1.0000 & 0.9960 \TBstrut\\ \hline
 %\rowcolor{grey}
%$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ1}^{DGA}$ & SN = 99.60\% , TN = 99.60\% & LBFGS, default parameter &  34.22 & 1.48 & 33.92 & 0.9930 & 0.6300 \TBstrut\\ \hline

\end{tabular}}
\end{table*}


==> Transactions-Bibliography/README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

IEEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************

